A Posteriori Error Estimation for the p-curl Problem

We derive a posteriori error estimates for a semi-discrete finite element approximation of a nonlinear eddy current problem arising from applied superconductivity, known as the $p$-curl problem. In particular, we show the reliability for non-conforming N\'{e}d\'{e}lec elements based on a residual type argument and a Helmholtz-Weyl decomposition of $W^p_0(\text{curl};\Omega)$. As a consequence, we are also able to derive an a posteriori error estimate for a quantity of interest called the AC loss. The nonlinearity for this form of Maxwell's equation is an analogue of the one found in the $p$-Laplacian. It is handled without linearizing around the approximate solution. The non-conformity is dealt by adapting error decomposition techniques of Carstensen, Hu and Orlando. Geometric non-conformities also appear because the continuous problem is defined over a bounded $C^{1,1}$ domain while the discrete problem is formulated over a weaker polyhedral domain. The semi-discrete formulation studied in this paper is often encountered in commercial codes and is shown to be well-posed. The paper concludes with numerical results confirming the reliability of the a posteriori error estimate.

==> SINUM arxiv/pcurlapee_info.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx,epstopdf}
\usepackage[caption=false]{subfig}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{A posteriori error estimation for the $p$-curl problem} 
\newcommand{\TheAuthors}{Andy T. S. Wan, and Marc Laforest}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{This work was supported by FQNRT, NSERC and MITACS.}}

% Authors: full names plus addresses.
\author{
  Andy T. S. Wan\thanks{Department of Mathematics and Statistics, University of Northern British Columbia, Prince George, British Columbia, Canada
    (\email{andy.wan@unbc.ca}).}
  \and
  Marc Laforest\thanks{d\'epartement de math\'ematiques et g\'enie industriel, \'Ecole Polytechnique de Montr\'eal, Montr\'eal, Qu\'ebec, Canada (\email{marc.laforest@polymtl.ca}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

\usepackage{amstext,amsfonts,amsmath,stmaryrd,amssymb}

\newsiamremark{hypothesis}{Hypothesis}

\providecommand{\norm}[1]{\left\lVert#1\right\rVert}
\providecommand{\pair}[1]{\langle#1\rangle_{\Omega}}
\providecommand{\pairh}[1]{\langle#1\rangle_{\Omega_h}}
\providecommand{\pairk}[1]{\langle#1\rangle_{K}}
\providecommand{\paire}[1]{\langle#1\rangle_{F}}
\providecommand{\rpair}[1]{\left(#1\right)_{\Omega}}
\providecommand{\rpairh}[1]{\left(#1\right)_{\Omega_h}}
\providecommand{\rpairk}[1]{\left(#1\right)_{K}}
\providecommand{\rpaire}[1]{\left(#1\right)_{F}}
\providecommand{\jump}[1]{\llbracket#1\rrbracket}
\providecommand{\Tau}{\mathcal{T}}

\newcommand{\bb}{\boldsymbol}
\renewcommand{\L}[1]{L^{#1}}
\newcommand{\Ldom}[1]{L^{#1}(\Omega)}
\newcommand{\Lbry}[1]{L^{#1}(\partial\Omega)}
\newcommand{\W}[1]{W^{#1,p}(\Omega)}
\newcommand{\Wz}{W_0^{1,p}(\Omega)}
\newcommand{\Wcurl}{W^p(\text{curl};\Omega)}
\newcommand{\Wcurlh}{W^p(\text{curl};\Omega_h)}
\newcommand{\Wzcurl}{W^p_0(\text{curl};\Omega)}
\newcommand{\Wzcurlh}{W^p_0(\text{curl};\Omega_h)}
\newcommand{\Wcurlz}{W^p(\text{curl}^0;\Omega)}
\newcommand{\Wdiv}{W^p(\text{div};\Omega)}
\newcommand{\Wzdiv}{W_0^p(\text{div};\Omega)}
\newcommand{\Wdivz}{W^p(\text{div}^0;\Omega)}
%\newcommand{\Wzdivz}{W_0^p(\text{div}^0;\Omega)}
\newcommand{\X}{V^p(\Omega)}
\newcommand{\Xq}{V^q(\Omega)}
\newcommand{\Xh}{V_{h}}
\newcommand{\Xhz}{V_{h,0}}
\newcommand{\curl}{\nabla\times}
\newcommand{\grad}{\nabla}
\renewcommand{\div}{\nabla\cdot}
\newcommand{\pdt}{\partial_t}
\newcommand{\param}{\alpha}

\newcommand{\aw}[1]{{\color{blue}#1}}

\newcommand{\Res}{\operatorname{Res}}
\newcommand{\Osc}{\operatorname{Osc}}
\newcommand{\NC}{\operatorname{NC}}
\newcommand{\Ext}{E_h}
\newcommand{\Extv}{E_h \bb{v}}
\newcommand{\intstrip}{\Omega_{h,i}}
\newcommand{\outstrip}{\Omega_{h,o}}

%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

